Joint Knowledge Base Completion and Question Answering by Combining Large Language Models and Small Language Models

Knowledge Bases (KBs) play a key role in various applications. As two representative KB-related tasks, knowledge base completion (KBC) and knowledge base question answering (KBQA) are closely related and inherently complementary with each other. Thus, it will be beneficial to solve the task of joint KBC and KBQA to make them reinforce each other. However, existing studies usually rely on the small language model (SLM) to enhance them jointly, and the large language model (LLM)'s strong reasoning ability is ignored. In this paper, by combining the strengths of the LLM with the SLM, we propose a novel framework JCQL, which can make these two tasks enhance each other in an iterative manner. To make KBC enhance KBQA, we augment the LLM agent-based KBQA model's reasoning paths by incorporating an SLM-trained KBC model as an action of the agent, alleviating the LLM's hallucination and high computational costs issue in KBQA. To make KBQA enhance KBC, we incrementally fine-tune the KBC model by leveraging KBQA's reasoning paths as its supplementary training data, improving the ability of the SLM in KBC. Extensive experiments over two public benchmark data sets demonstrate that JCQL surpasses all baselines for both KBC and KBQA tasks.

==> tables/Effect_Analysis_of_the_generated_triples_for_KGQA_inference..tex <==
\renewcommand{\arraystretch}{1.5}
\begin{table*}[ht!]
\centering
\begin{tabular}{>{\hspace{0pt}}m{0.1\linewidth}|>{\hspace{0pt}}m{0.9\linewidth}} 
\hline
\rowcolor[rgb]{0.9490,0.9490,0.9490} Train     & Question: What language with the initials fra is spoken in Haiti?\par{}Topic Entity: [Haiti]\par{}Reference answer: French\par\null\par{}Thought 1:~The task requires identifying the language spoken in Haiti that has the initials "fra" Since French is the official language of Haiti, I will focus on gathering information about languages spoken in Haiti.\par{}Action 1:~Search[Haiti]\par{}Observation 1:~Haiti, language used, Haitian Creole\par{}Haiti, language used, Haitian Vodoun Culture Language\par{}Haiti, official language, Haitian Creole\par{}Tahiti, different from, Haiti\par\null\par{}Thought 2:~The search results indicate that Haitian Creole is commonly used in Haiti, but they do not mention French. However, I know that French is also an official language of Haiti. I need to confirm this by checking what languages are officially recognized in Haiti.\par{}Action 2:~\textcolor[rgb]{0.7529,0,0}{Generate[what are the official languages of Haiti?]}\par{}Observation 2: \textcolor[rgb]{0.4549,0.7137,0.0078}{Haiti, official language, French}\par{}\textcolor[rgb]{0.4549,0.7137,0.0078}{Haiti, language used, French}\par{}Haiti, official language, Haitian Creole\par\null\par{}Thought 3:~The generated results confirm that French is indeed one of the official languages of Haiti along with Haitian Creole. Since I need to identify the language with the initials "fra" and I have confirmed that French is recognized as an official language, I can finalize my answer.\par{}Action 3:~Finish[French]  \\
\hline
\rowcolor[rgb]{0.9490,0.9490,0.9490} Inference  & Question: The people from the country that contains Nord-Ouest Department speak what languages today?\par{}Topic Entity: [Nord-Ouest Department]\par\null\par{}Thought 1:~I need to determine which country contains the Nord-Ouest Department to find out the languages spoken there.\par{}Action 1:~Search[Nord-Ouest Department]\par{}Observation 1:~Artibonite, shares border with, Nord-Ouest\par{}Haiti, contains the administrative territorial entity, Nord-Ouest\par{}Nord-Ouest, category for people born here, wd:Q107541733\par\null\par{}Thought 2:~The Nord-Ouest Department is located in Haiti. Now, I need to find out what languages are spoken in Haiti to answer the question about the languages spoken in the Nord-Ouest Department.\par{}Action 2:~Search[Haiti]\par{}Observation 2: Haiti, has part(s), North America\par{}\textcolor[rgb]{0.4549,0.7137,0.0078}{Haiti, language used, French}\par{}Haiti, language used, Haitian Creole\par{}Haiti, language used, Haitian Vodoun Culture Language\par{}\textcolor[rgb]{0.4549,0.7137,0.0078}{Haiti, official language, French}\par{}Haiti, official language, \textcolor[rgb]{0,0.4392,0.7529}{Haitian Creole}\par{}Latin America, has part(s), Haiti\par{}North America, has part(s), Haiti\par\null\par{}Thought 3:~The search results indicate that the languages spoken in Haiti include French and Haitian Creole. To summarize, I need to confirm these findings and present them clearly.\par{}Action 3:~Finish[\textcolor[rgb]{0,0.4392,0.7529}{French} | \textcolor[rgb]{0,0.4392,0.7529}{Haitian Creole}]  \\
\hline
\end{tabular}
\caption{Effect Analysis of the generated triples for KBQA inference. The \textcolor[rgb]{0.7529,0,0}{Generate action} are highlighted with red color, The \textcolor[rgb]{0.4549,0.7137,0.0078}{generated triples} are highlighted with green color, and the \textcolor[rgb]{0,0.4392,0.7529}{correct answers} are highlighted with blue color.}
\label{tab:cmp_t5}
\end{table*}
\renewcommand{\arraystretch}{1}
